S3-Net: A Fast and Lightweight Video Scene Understanding Network by Single-shot Segmentation

Real-time understanding in video is crucial in various AI applications such as autonomous driving. This work presents a fast single-shot segmentation strategy for video scene understanding. The proposed net, called S3-Net, quickly locates and segments target sub-scenes, meanwhile extracts structured time-series semantic features as inputs to an LSTM-based spatio-temporal model. Utilizing tensorization and quantization techniques, S3-Net is intended to be lightweight for edge computing. Experiments using CityScapes, UCF11, HMDB51 and MOMENTS datasets demonstrate that the proposed S3-Net achieves an accuracy improvement of 8.1% versus the 3D-CNN based approach on UCF11, a storage reduction of 6.9x and an inference speed of 22.8 FPS on CityScapes with a GTX1080Ti GPU.

==> sections/ttalgorithm.tex <==
\begin{algorithm}[hbt] \small
\caption{Training SU-Net with tensorization and quantization.}
\label{alg:algorithm}
\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Require:}}
\renewcommand{\algorithmicensure}{\textbf{Ensure:}}
\begin{algorithmic}[1]
\REQUIRE Frame tensor data $\bm{\mathcal{F}}$, bias vector $\bm{b}$, number of fully-connected layers $L$, dimensional $d$, mode size of tensors $l_1,l_2,\cdots,l_d$ and ranks $r_1, \cdots, r_{d-1}$.
\ENSURE Training accuracy $\bm{P}$.\\

\STATE Feed $\bm{F}$ into the trained feature extractor
\STATE Obtain tensor feature outputs $\bm{\mathcal{X}}$
\FOR{$k=1:L$}
%\IF{d==2}
%\STATE Factorize $l_1$ and $l_2$ (e.g. $n_{1}\times m_{1}\leftarrow l_1$ and $n_{2}\times m_{2}\leftarrow l_2$)
%\STATE $\bm{\mathcal{W}}_k\leftarrow reshape(\bm{W}_k)$
%\STATE $\bm{{X}}, \bm{{B}} \leftarrow reshape(\bm{x}, \bm{b})$
%\STATE Generate tensor cores $\bm{\mathcal{G}}^t_1 \in \mathbb{R}^{n_1\times m_1 \times r_1 \times 1}$ and $\bm{\mathcal{G}}^t_2 \in \mathbb{R}^{n_2\times m_2 \times 1 \times r_1}$ to represent the weight tensor $\bm{\mathcal{W}}_k \in \mathbb{R}^{n_1\times n_2\times m_1\times m_2}$: $\bm{\mathcal{G}}^t_1\bm{\mathcal{G}}^t_2 \leftarrow \bm{\mathcal{W}}_k $
%\STATE $\bm{\mathcal{G}}^q, \bm{{X}}^q, \bm{{B}}^q \leftarrow quantize(\bm{\mathcal{G}}, \bm{{X}}, \bm{{B}})$
%\STATE $\bm{{Y}}^q\leftarrow compute(\bm{\mathcal{G}}_k^{tq}, \bm{{X}}^q, \bm{{B}}^q)$
%\ELSE
\STATE Factorize $l_1,l_2,\cdots, l_d$ by: $n_{1}\times m_{1}\leftarrow l_1$, $n_{2}\times m_{2}\leftarrow l_2$,$\cdots$, $n_{d}\times m_{d}\leftarrow l_d$
\STATE $\bm{\mathcal{W}}_k, \bm{\mathcal{B}} \leftarrow reshape(\bm{W}_k, \bm{b})$
%\STATE Generate tensor cores $\bm{\mathcal{G}}^t_1 \in \mathbb{R}^{n_1\times m_1 \times r_1 \times 1}$, $\bm{\mathcal{G}}^t_2 \in \mathbb{R}^{n_2\times m_2 \times r_2 \times r_1}$, $\cdots$, $\bm{\mathcal{G}}^t_d \in \mathbb{R}^{n_d\times m_d \times 1 \times r_{d-1}}$ based on Eq.~(\ref{eq:tensor4})
\STATE Decompose $\bm{\mathcal{W}}_k$ into tensor cores: $\bm{\mathcal{G}}^t_1\bm{\mathcal{G}}^t_2\cdots \bm{\mathcal{G}}^t_d \leftarrow \bm{\mathcal{W}}_k $
%\STATE Decompose $\bm{\mathcal{W}}_k$ to $d$ tensor cores based on Eq.~(\ref{eq:tensor4})
\STATE $\bm{\mathcal{G}}^q, \bm{\mathcal{X}}^q, \bm{\mathcal{B}}^q \leftarrow quantize(\bm{\mathcal{G}}, \bm{\mathcal{X}}, \bm{\mathcal{B}})$
\STATE $\bm{\mathcal{Y}}^q\leftarrow compute(\bm{\mathcal{G}}^{q}, \bm{\mathcal{X}}^q, \bm{\mathcal{B}}^q)$
%\ENDIF
\ENDFOR
\STATE Get the training accuracy $\bm{P}$
\IF{$\bm{P}$ is satisfactory}
\STATE Save the trained model
\STATE Run scene segmentation and understanding
\ELSE
\STATE Increase $L$ and repeat Steps 1,2 and 3
\ENDIF
\end{algorithmic}
\end{algorithm}

